Automatic latency balancing in VHDL-implemented complex pipelined systems

Balancing (equalization) of latency in parallel paths in the pipelined data processing system is an important problem. Without that the data from different paths arrive at the processing blocks in different clock cycles, and incorrect results are produced. Manual correction of latencies is a tedious and error-prone work. This paper presents an automatic method of latency equalization in systems described in VHDL. The method is based on simulation and is portable between different simulation and synthesis tools. The method does not increase the complexity of the synthesized design comparing to the solution based on manual latency adjustment. The example implementation of the proposed methodology together with a simple design demonstrating its use is available as an open source project under BSD license.

==> rysunki.src/makefile <==
.SUFFIXES: .svg .dia .fig .eps .figmp .figltx .pdf .jpg .drt .ipe .png .odg
EPS := $(patsubst %.fig,%.eps,$(wildcard *.fig))\
 $(patsubst %.figmp,%.eps,$(wildcard *.figmp))\
 $(patsubst %.figltx,%.eps,$(wildcard *.figltx))\
 $(patsubst %.pdf,%.eps,$(wildcard *.pdf)) \
 $(patsubst %.svg,%.eps,$(wildcard *.svg)) \
 $(patsubst %.dia,%.eps,$(wildcard *.dia)) \
 $(patsubst %.drt,%.eps,$(wildcard *.drt)) \
 $(patsubst %.ipe,%.eps,$(wildcard *.ipe)) \
 $(patsubst %.png,%.eps,$(wildcard *.png)) \
 $(patsubst %.odg,%.eps,$(wildcard *.odg)) \
 $(patsubst %.jpg,%.eps,$(wildcard *.jpg))
  

all: $(EPS) $(DIAEPS)
	echo $(EPS)
	echo Rysunki przetworzone

.jpg.eps: *.jpg
#       jpeg2ps $*.jpg > ../rysunki/$*.eps
	sam2p -3 -c:jpeg $*.jpg  ../rysunki/$*.eps
	ln -s -f ../rysunki.src/$*.jpg ../rysunki/$*.jpg

.odg.eps: *.odg
#       jpeg2ps $*.jpg > ../rysunki/$*.eps
	lodraw --headless --convert-to eps --outdir ../rysunki $*.odg
	lodraw --headless --convert-to pdf --outdir ../rysunki $*.odg

.png.eps: *.png
#       jpeg2ps $*.jpg > ../rysunki/$*.eps
	sam2p -3 -c:lzw $*.png  ../rysunki/$*.eps
	sam2p -3 -c:lzw $*.png  ../rysunki/$*.pdf

.fig.eps: *.fig
	fig2dev -L eps $*.fig  ../rysunki/$*.eps
	fig2dev -L pdf $*.fig  ../rysunki/$*.pdf

.pdf.eps: *.pdf
	pdftops -eps $*.pdf  ../rysunki/$*.eps
	ln -s -f $*.pdf ../rysunki/$*.pdf

.figmp.eps: *.figmp
	fig2dev -L mp $*.figmp ../rysunki.tmp/$*.mp
	( cd ../rysunki.tmp ; mpost $*.mp )
	mv ../rysunki.tmp/$*.0 ../rysunki/$*.eps

.figltx.eps: *.figltx
	fig2dev -L pstex -p rysunki/$*.eps $*.figltx ../rysunki/$*.eps
	fig2dev -L pstex_t -p rysunki/$*.eps $*.figltx ../rysunki/$*.tex

.dia.pdf: *.dia
	dia --nosplash -e ../rysunki/$*.pdf -t pdf $*.dia

.dia.eps: *.dia
	dia --nosplash -e ../rysunki/$*.eps -t eps-builtin $*.dia

.drt.eps: *.drt
	drawtiming --output ../rysunki/$*.eps $*.drt

.ipe.eps: *.ipe
	ipetoipe -eps -export $*.ipe ../rysunki/$*.eps

.svg.eps: *.svg
	inkscape -z  -E../rysunki/$*.eps -f $*.svg
#	inkscape -z -d 600 -E../rysunki/$*.eps -f $*.svg
#	inkscape -z --export-ignore-filters -E../rysunki/$*.eps -f $*.svg
	

